Uncertainty-Based Knowing How Logic

We introduce a novel semantics for a multi-agent epistemic operator of knowing how, based on an indistinguishability relation between plans. Our proposal is, arguably, closer to the standard presentation of knowing that modalities in classical epistemic logic. We study the relationship between this new semantics and previous approaches, showing that our setting is general enough to capture them. We also study the logical properties of the new semantics. First, we define a sound and complete axiomatization. Second, we define a suitable notion of bisimulation and prove correspondence theorems. Finally, we investigate the computational complexity of the model checking and satisfiability problems for the new logic.

==> modelequiv.tex <==
%!TEX root = main.tex

\subsection{Active and compositional \ultss} \label{subsec:active-compositional}

We presented above a very simple class of models that enables us to establish a direct relation between both semantics. However, the result is quite obvious as \ultss are a generalization of \ltss, and what we did it to restrict ourselves to those \ultss that behave in fact as \ltss. One may wonder whether a more general class can be defined, for which the same correspondence holds.

A larger class can be defined by asking directly for what \axm{EMP} and \axm{COMPKh} require: a set of plans that plays $\epsilon$'s role (there is $\strategy_\epsilon \in \S$ with $\R_{\strategy_\epsilon} = \R_\epsilon$) and closure of $\S$ under composition ($\strategy_1, \strategy_2 \in \S$ imply there is $\strategy_{\strategy_1\strategy_2} \in \S$ such that $\R_{\strategy_{\strategy_1\strategy_2}} = \R_{\strategy_1} \circ \R_{\strategy_2}$) (where `$\circ$' denotes the standard composition of relations).
This is clearly a larger class: any $\ults$ satisfying $\DS{} = \ACT^*$ and $\S = \csetsc{\cset{\sigma}}{\sigma \in \DS{}}$ fulfils both requirements. In the rest of this section we will go a bit further, and will define a very general class (with very weak constraints) satisfying the above-mentioned conditions. 

Let us start by introducing some preliminary definitions. 

\begin{definition} \label{def:composition}
  Let $\model=\tup{\W,\R,\S,\V}$ be an $\ults$. We define the \emph{composition} of $\strategy_1,\strategy_2\in \S$ as
  %\begin{nscenter}
      \begin{equation*}
          \strategy_1 \compose \strategy_2 : =
          \begin{cases*}
             \{\sigma_1\sigma_2 \mid \sigma_1\in\strategy_1 \mbox{ and } \sigma_2\in\strategy_2\} & if $\stexec(\strategy_1)\neq \emptyset$ and $\R_{\strategy_1}(\stexec(\strategy_1))\subseteq \stexec(\strategy_2)$ \\
            \emptyset        & otherwise.
          \end{cases*}
        \end{equation*}
%
    % $\begin{array}{ll}
    % \strategy_1 \compose \strategy_2 := &  \{\sigma_1\sigma_2 \mid 
    % \sigma_1\in\strategy_1,~\sigma_2\in\strategy_2, \R_{\sigma_1}(\W)\neq\emptyset,\text{ and } \R_{\sigma_1}(\W) \subseteq \stexec(\sigma_2) \}.
    % \end{array}$
  %\end{nscenter}
\end{definition}

% Thus, a plan is in $\strategy_1 \compose \strategy_2$ if and only if
% it is the sequential composition of some plans $\sigma_1\in\strategy_1$ and $\sigma_2\in\strategy_2$ (in that order) such that  $\sigma_1$ is executable (i.e., there is some state reached from executing $\sigma_1$) and in all the states reached by executing $\sigma_1$, the plan $\sigma_2$ is strongly executable.

Thus, $\strategy_1 \compose \strategy_2$ contains the sequential composition $\sigma_1\sigma_2$ of plans $\sigma_1\in\strategy_1$ and $\sigma_2\in\strategy_2$ when $\strategy_1$ is strongly executable somewhere in the model and $\strategy_2$ is strongly executable at those states reachable via $\strategy_1$. Otherwise, $\strategy_1 \compose \strategy_2=\emptyset$, thus guaranteeing that the composition succeeds only for suitable sets of plans. 

Let us introduce the following properties over $\ults${s}.

\begin{definition}\label{def:esm-req}
  We say that an $\ults$ $\model=\tup{\W,\R,\S,\V}$ is:
  \begin{itemize}
  \item \emph{active} {\siffdefs} there exists $\strategy\in\S$ s.t.
    $\stexec(\strategy)=\W$ and, for all $u,v\in\W$,
    $v\in\R_{\strategy}(u)$ implies $\model,u\bisim\model,v$.

    This ensures that $\strategy \in \S$ behaves as the empty plan
    $\epsilon$ does in an \lts.

  \item \emph{compositional} {\siffdefs} for all
    $\strategy_1,\strategy_2\in\S$ with 
    $\strategy_1\compose\strategy_2\neq\emptyset$ there exists
    $\strategy\in\S$ s.t.:
    \begin{enumerate} 
      \item $\R_{\strategy_1\compose\strategy_2}\subseteq \R_{\strategy}$, and 
      \item for all $(w,v) \in \R_\strategy$, there exists
            $(w',v')\in\R_{\strategy_1\compose\strategy_2}$, such that 
            $\model,w\bisim\model,w'$ and 
            $\model,v\bisim\model,v'$.
    \end{enumerate}
    This ensures that $\S$ is closed under a suitable notion of
    composition of strategies.
  \end{itemize}
\end{definition}

Notice that by asking bisimilarity between the states that are related by the corresponding sets of plans, we relax a bit our constraints and obtain a slightly more general class of models.

Now, we will show that for every \lts there is an $\KHlogic$-equivalent
active and compositional $\ults$ and vice-versa. First, we present the
mapping from $\ultss$ to \ltss.

\begin{proposition}\label{prop:esmtolts}
  Let $\model=\tup{\W,\R,\S,\V}$ be an active and compositional $\ults$
  over $\ACT$. Let
  $\ACT' := \csetsc{a_{\strategy}}{\strategy \in \S }$. Define the \lts
  $\modlts_{\model} = \tup{\W, \R', \V}$ over $\ACT'$, where
  $\R'_{a_{\strategy}} := \R_{\strategy}$ (so basic actions in
  $\modlts_\model$ correspond to set of plans in $\model$). Then, for every
  $\varphi \in \KHlogic$, we have
  $\truthset{\model}{\varphi} = \truthset{\modlts_\model}{\varphi}$.
\end{proposition}

\begin{proof}
  The proof is by structural induction on the formulas in $\KHlogic$.
  The cases for the Boolean fragment are straightforward.  We will
  discuss the case for formulas of the shape $\kh(\psi,\varphi)$.

  \ssparagraph{$\boldsymbol{(\Rightarrow)}$} Suppose
  $w \in \truthset{\model}{\kh(\psi,\varphi)}$; then there is
  $\strategy \in \S \subseteq 2^{(\ACT^*)}$
  satisfying 
  \begin{enumerate}
    \item\label{pro1:lr:itm:i}
    $\truthset{\model}{\psi} \subseteq \stexec(\strategy)$
    and 
    \item\label{pro1:lr:itm:ii}
    $\R_\strategy(\truthset{\model}{\psi}) \subseteq
    \truthset{\model}{\varphi}$.
  \end{enumerate}
    %First, note how plan
  %$a_{\strategy} \in \ACT'$ (and thus in $(\ACT')^*$) satisfies the SE 
  %requirement \emph{in $\lts$}.
  Suppose $v \in \truthset{\modlts_\model}{\psi}$; by IH, 
  $v \in \truthset{\model}{\psi}$.  By item~\ref{pro1:lr:itm:i}, we
  have $v \in \stexec(\strategy)$, and by definition of $\stexec$,
  $\R_{\strategy}(v) \neq \emptyset$. Hence,
  $\R'_{a_{\strategy}}(v) \neq \emptyset$ (by definition of $\R'$), and
  since $a_{\strategy}$ is a basic action,
  $a_{\strategy} \;\text{is SE at } v$. Thus,
  $v \in \stexec(a_{\strategy})$, and therefore
  $\truthset{\modlts_\model}{\psi} \subseteq \stexec(a_\strategy)$.

  Now, we show that $a_{\strategy}$ does the required work. Suppose
  $u \in \R'_{a_{\strategy}}(\truthset{\modlts_\model}{\psi})$; by
  IH, $u \in \R'_{a_{\strategy}}(\truthset{\model}{\psi})$, then $u \in
  \R_{\strategy}(\truthset{\model}{\psi})$ (by
  definition of $\R'$). Then, by item~\ref{pro1:lr:itm:ii}, $u \in \truthset{\model}{\varphi}$, and
  by IH $u \in \truthset{\modlts_\model}{\varphi}$.  Thus, we have
  $\R'_{a_{\strategy}}(\truthset{\modlts_\model}{\psi}) \subseteq
  \truthset{\modlts_\model}{\varphi}$.  Hence,
  $w \in \truthset{\modlts_\model}{\kh(\psi,\varphi)}$.
    

  \ssparagraph{$\boldsymbol{(\Leftarrow)}$} Suppose
  $w \in \truthset{\modlts_\model}{\kh(\psi,\varphi)}$; then there is
  $\sigma \in (\ACT')^*$ satisfying 
  \begin{enumerate}
    \item\label{pro1:rl:itm:i} $\truthset{\modlts_\model}{\psi} \subseteq \stexec(\sigma)$
    and \item\label{pro1:rl:itm:ii}
    $\R'_\sigma(\truthset{\modlts_\model}{\psi}) \subseteq
    \truthset{\modlts_\model}{\varphi}$.
  \end{enumerate}
   There are two
  cases. First, assume $\sigma=\epsilon$. Since $\model$ is active, there is
  $\strategy\in\S$ s.t. for all $u,v\in\W$, $v\in\R_{\strategy}(u)$
  implies $\model,u\bisim\model,v$; this is the witness we need.
    %
    %% Keep the text below for a long version of the paper
    %
    % \begin{enumerate}[\bfseries \itshape (i')]
    %   \item Take any $u \in \W$; note how $\R_\epsilon (u) \neq \emptyset$. Moreover, from $\epsilon \in \strategy$ it follows that $\R_\epsilon (u) \subseteq \R_\strategy (u)$. Hence, $\R_\strategy (u) \neq \emptyset$ (i.e., $u \in \stexec(\strategy)$) for all $u \in \W$, and thus in particular for every $u \in \truthset{\model}{\psi}$. Therefore, $\truthset{\model}{\psi} \subseteq \stexec(\strategy)$. 
    %  
    %   \item Since $\sigma = \epsilon$, we have $\R'_\sigma(\truthset{\modlts_\model}{\psi}) = \truthset{\modlts_\model}{\psi}$; hence, \ref{pro1:rl:itm:ii} above actually says $\truthset{\modlts_\model}{\psi} \subseteq \truthset{\modlts_\model}{\varphi}$. Moreover, from $\strategy$'s constrains, $(u,v) \in \R_{\strategy}$ implies $u,v$ are bisimilar, so (\ref{th:khbisim-to-khequiv}) both satisfy exactly the same formulas in $\model$. Thus, $u \in \R_\strategy(\truthset{\model}{\psi})$ implies $u \in \truthset{\model}{\psi}$ (condition on $\strategy$), which implies $u \in \truthset{\modlts_\model}{\psi}$ (IH), which implies $u \in \truthset{\modlts_\model}{\varphi}$ (see above), which implies $u \in \truthset{\model}{\varphi}$ (IH). Hence, $\R_\strategy(\truthset{\model}{\psi}) \subseteq \truthset{\model}{\varphi}$.
    % \end{enumerate}
    % Hence, $w \in \truthset{\model}{\kh(\psi,\varphi)}$.
    %        
    % {\smallskip}
    Second, assume $\sigma\neq\epsilon$, i.e., $\sigma=a_{\strategy_1}{\cdots}a_{\strategy_k}$ with $a_{\strategy_i} \in \ACT'$ (so $\strategy_i \in \S$). Then, we have two cases:
    \begin{itemize}
      \item  If $\strategy_1 ; \cdots ; \strategy_k = \emptyset$, there exists $0<i\leq k$ s.t. $\strategy_i\compose\strategy_{i+1}=\emptyset$. Then (by Definition~\ref{def:composition}), either $\stexec(\strategy_i)=\emptyset$ and thus $\stexec(a_{\strategy_i})=\emptyset$; or $\R_{\strategy_i}(\stexec(\strategy_i)\not\subseteq\stexec(\strategy_{i+1})$, which implies 
      $\R'_{a_{\strategy_i}}(\stexec(a_{\strategy_i}))\not\subseteq\stexec(a_{\strategy_{i+1}})$.
      In both cases we get that $\stexec(\sigma)=\emptyset$, and hence, $\truthset{\modlts_\model}{\psi} = \emptyset$ (by item \ref{pro1:rl:itm:i}). By IH, this implies $\truthset{\model}{\psi} = \emptyset$, so to get $w \in \truthset{\modlts_\model}{\kh(\psi,\varphi)}$ we only need $\S \neq \emptyset$, which we have as $\model$ is an $\ults$.
    
      \item If $\strategy_1 ; \cdots ; \strategy_k \neq \emptyset$, take $u \in \R_{\strategy}(\truthset{\model}{\psi})$. Thus, $(v,u) \in \R_{\strategy}$ for $v \in \truthset{\model}{\psi}$. Since $\model$ is compositional, by Definition~\ref{def:composition} and a simple induction on $k$, there exists $\strategy\in\S$ such that $\R_{\strategy_1;\cdots;\strategy_k}\subseteq\R_\strategy$, and for all $(v,u) \in \R_{\strategy}$, we have $(v',u') \in \R_{\strategy_1;\cdots;\strategy_k}$ for some $v', u' \in \W$ satisfying $\model,u\bisim\model,u'$ and $\model,v\bisim\model,v'$. Then, $(v',u') \in \R_{\strategy_1;\cdots;\strategy_k}$ for $v' \in \truthset{\model}{\psi}$, and as consequence, $u' \in \R_{\strategy_1;\cdots;\strategy_k}(\truthset{\model}{\psi})$. By IH, we have $u' \in \R_{\strategy_1;\cdots;\strategy_k}(\truthset{\modlts_\model}{\psi})$, or equivalently, $u' \in (\R_{\strategy_1} \circ \cdots \circ \R_{\strategy_k})(\truthset{\modlts_\model}{\psi})$. By definition of $\R'$, we obtain that $u' \in (\R'_{a_{\strategy_1}} \circ \cdots \circ \R'_{a_{\strategy_k}})(\truthset{\modlts_\model}{\psi})$, hence $u' \in \R'_{a_{\strategy_1}{\cdots}a_{\strategy_k}}(\truthset{\modlts_\model}{\psi})$. Thus, by item~\ref{pro1:rl:itm:ii} we get $u' \in \truthset{\modlts_\model}{\varphi}$, and by IH, $u' \in \truthset{\model}{\varphi}$. Therefore, $u \in \truthset{\model}{\varphi}$ (as $\model,u\bisim\model,u'$, and by Theorem~\ref{th:khbisim-to-khequiv}).                                          
      
      
      % To prove that
      % $\R_{\strategy}(\truthset{\model}{\psi}) \subseteq \truthset{\model}{\varphi}$,
      % we can follow .
      %%
      % Keep the text below for a long version
      %
      % Then,
      % \begin{enumerate}[\bfseries \itshape (i')]
      %   \item \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
      %           $u \in \truthset{\model}{\psi}$ & $u \in \truthset{\modlts_\model}{\psi}$                                                        & IH \\
      %                                           & $u \in \stexec(\sigma)$                                                              & \ref{pro1:rl:itm:i} \\
      %                                           & $u \in \stexec(a_{\strategy_1}{\cdots}a_{\strategy_k})$                              \\
      %                                           & $\R'_{a_{\strategy_1}{\cdots}a_{\strategy_k}}(u) \neq \emptyset$                     & definition of $\mathit{SE}$ \\
      %                                           & $(\R'_{a_{\strategy_1}} \circ \cdots \circ \R'_{a_{\strategy_k}})(u) \neq \emptyset$ \\
      %                                           & $(\R_{\strategy_1} \circ \cdots \circ \R_{\strategy_k})(u) \neq \emptyset$           & definition of $\R'$ \\
      %                                           & $\R_{\strategy_1;{\cdots};\strategy_k}(u) \neq \emptyset$                            \\
      %                                           & $\R_{\strategy}(u) \neq \emptyset$                                                   & \footnotemark \\
      %                                           & $u \in \stexec(\strategy)$                                                             \\
      %         \end{tabular}
      %   \footnotetext{By compositionality and $\strategy_1 ; \cdots ; \strategy_k \neq \emptyset$, the given $\strategy$ is such that $\strategy_1 ; \cdots ; \strategy_k \subseteq \strategy$.}
        
      %   Thus, $\truthset{\model}{\psi} \subseteq \stexec(\strategy)$.

      %   \item \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
      %           $u \in \R_{\strategy}(\truthset{\model}{\psi})$ & $(v,u) \in \R_{\strategy}$ for $v \in \truthset{\model}{\psi}$                                  \\
      %                                                           & $(v',u') \in \R_{\strategy_1;\cdots;\strategy_k}$ for $v' \in \truthset{\model}{\psi}$          & \footnotemark \\
      %                                                           & $u' \in \R_{\strategy_1;\cdots;\strategy_k}(\truthset{\model}{\psi})$                           \\
      %                                                           & $u' \in \R_{\strategy_1;\cdots;\strategy_k}(\truthset{\modlts_\model}{\psi})$                              & IH \\
      %                                                           & $u' \in (\R_{\strategy_1} \circ \cdots \circ \R_{\strategy_k})(\truthset{\modlts_\model}{\psi})$           \\
      %                                                           & $u' \in (\R'_{a_{\strategy_1}} \circ \cdots \circ \R'_{a_{\strategy_k}})(\truthset{\modlts_\model}{\psi})$ & definition of $\R'$ \\
      %                                                           & $u' \in \R'_{a_{\strategy_1}{\cdots}a_{\strategy_k}}(\truthset{\modlts_\model}{\psi})$                     \\
      %                                                           & $u' \in \truthset{\modlts_\model}{\varphi}$                                                                & \ref{pro1:rl:itm:ii} \\
      %                                                           & $u' \in \truthset{\model}{\varphi}$                                                              & IH \\
      %                                                           & $u \in \truthset{\model}{\varphi}$                                                               \\
      %         \end{tabular}
%     By compositionality and $\strategy_1 ; \cdots ; \strategy_k \neq \emptyset$, the given $\strategy$ is such that $(v,u) \in \R_{\strategy}$ implies $(v',u') \in \R_{\strategy_1;\cdots;\strategy_k}$ for some $v', u' \in \W$ satisfying $\model,u\bisim\model,u'$ and $\model,v\bisim\model,v'$.
 %             
      %   Then, $\R_{\strategy}(\truthset{\model}{\psi}) \subseteq \truthset{\model}{\varphi}$.
      % \end{enumerate}
   \end{itemize}
   Hence, $w \in \truthset{\model}{\kh(\psi,\varphi)}$.      
  \end{proof}


  Now we will prove the other direction. From an \lts we can obtain an
  active and compositional $\ults$ satisfying the same formulas. This
  result will be useful to show completeness later on.

\begin{proposition}\label{prop:ltstoesm}
  Let $\modlts=\tup{\W,\R,\V}$ be an \lts over $\ACT$. Take
  $\ACT' := \csetsc{a_{\sigma}}{\sigma \in \ACT^* \;\text{and}\;
    \stexec(\sigma) \neq \emptyset }$. We define $\model_{\modlts} = \tup{\W,\R', \S', \V}$ over $\ACT'$ by taking
  $\R'_{a_{\sigma}} := \csetsc{(u,v) \in \W \times \W}{u \in
    \stexec(\sigma) \;\text{and}\; v \in \R_{\sigma}(u)}$ (so basic
  actions in $\model_{\modlts}$ are strongly executable plans in
  $\modlts$) and $\S':=\csetsc{\cset{a_\sigma}}{a_\sigma \in
    \ACT'}$. Then,
  \begin{enumerate}
    \item $\model_{\modlts}$ is an active and compositional $\ults$;
    \item for every $\varphi \in \KHlogic$, 
    $\truthset{\modlts}{\varphi} = \truthset{\model_{\modlts}}{\varphi}$.
  \end{enumerate}
\end{proposition}

  \begin{proof}
    (1) Note: $\S'$ is non-empty ($\epsilon\in\ACT^*$ and is SE everywhere, so $\epsilon \in \ACT'$ and hence $\cset{a_{\epsilon}} \in \S'$) and its elements are pairwise disjoint. Thus, $\model_{\modlts}$ is an $\ults$. Activeness is straightforward, as $\cset{a_\epsilon} \in \S'$,
    and it behaves exactly as $\epsilon$. 
    
    For compositionality, take $\cset{a_{\sigma_1}}, \cset{a_{\sigma_2}}\in\S'$ 
    s.t. $\cset{a_{\sigma_1}}\compose \cset{a_{\sigma_2}}\neq\emptyset$, i.e.,
    for all $v\in\R'_{a_{\sigma_1}}(\stexec(a_{\sigma_1}))$, $v\in\stexec(a_{\sigma_2)}$ ($\otimes_1$).
    As this is the case, then $\cset{a_{\sigma_1}}\compose \cset{a_{\sigma_2}}=\cset{a_{\sigma_1}a_{\sigma_2}}$. We need to check that there exists 
    $\strategy\in\S'$ satisfying the compositionality conditions. We propose 
    to take $\strategy=\cset{a_{\sigma_1\sigma_2}}$ as such strategy.
    
   First, we need to prove $\R'_{a_{\sigma_1}a_{\sigma_2}}\subseteq\R'_{a_{\sigma_1\sigma_2}}$. Suppose $(w,v)\in\R'_{a_{\sigma_1}a_{\sigma_2}}$. 
  Then, $w\in\stexec(a_{\sigma_1})$ and there exists $u\in\W$ s.t. $(w,u)\in\R'_{a_{\sigma_1}}$ and $(u,v)\in\R'_{a_{\sigma_2}}$. %Notice that by ($\otimes_1$),   $u\in\stexec(a_{\sigma_2)}$. 
  By definition of $\R'$, $(w,u)\in\R_{\sigma_1}$ and $(u,v)\in\R_{\sigma_2}$, then we have 
  $(w,v)\in\R_{\sigma_1\sigma_2}$. It remains to show that $\stexec(\sigma_1\sigma_2)\neq\emptyset$. We know that $w\in\stexec(a_{\sigma_1})$, 
  then $w\in\stexec(\sigma_1)$. Also, by ($\otimes_1$), for all $u\in\R'_{a_{\sigma_1}}(w)$, $u\in\stexec(a_{\sigma_2})$, which by construction of $\R'$ 
  implies that for all $u\in\R_{\sigma_1}(w)$, $u\in\stexec(\sigma_2)$.
  Then, $w\in\stexec(\sigma_1\sigma_2)$, which implies $a_{\sigma_1\sigma_2}\in\ACT'$. Thus, $(w,v)\in\R'_{a_{\sigma_1\sigma_2}}$.

    In a similar way, it can be shown that $\R'_{a_{\sigma_1\sigma_2}}\subseteq\R'_{a_{\sigma_1}a_{\sigma_2}}$ (as a consequence $\R'_{a_{\sigma_1\sigma_2}}=\R'_{a_{\sigma_1}a_{\sigma_2}}$). Thus, the second compositionality 
    condition is direct.

    {\medskip}
    
    (2) The proof is by structural induction; again, only the case of
    $\kh(\psi,\varphi)$ is discussed.
      
    \ssparagraph{$\boldsymbol{(\Rightarrow)}$} Suppose $w \in \truthset{\modlts}{\kh(\psi,\varphi)}$; then there is $\sigma \in \ACT^*$ satisfying 
    \begin{enumerate}
       \item\label{pro2:lr:itm:i} $\truthset{\modlts}{\psi} \subseteq \stexec(\sigma)$ and 
       \item\label{pro2:lr:itm:ii} $\R_\sigma(\truthset{\modlts}{\psi}) \subseteq \truthset{\modlts}{\varphi}$.
      \end{enumerate}
       There are two cases.
    
%    {\smallskip}
    
    First, assume $\stexec(\sigma)=\emptyset$. From this, item~\ref{pro2:lr:itm:i} implies $\truthset{\modlts}{\psi} = \emptyset$, so for $w \in \truthset{\model_{\modlts}}{\kh(\psi,\varphi)}$ it is enough to have $\S' \neq \emptyset$, which we do as $\cset{a_{\epsilon}} \in \S'$.
    
    %{\smallskip}
    
    Second, assume $\stexec(\sigma) \neq \emptyset$. Then, $a_\sigma \in \ACT'$ and $\cset{a_\sigma} \in \S'$. Take $\strategy = \cset{a_\sigma}$ as our witness.
    Suppose $u \in \truthset{\model_{\modlts}}{\psi}$, then by IH $u \in \truthset{\modlts}{\psi}$. By item~\ref{pro2:lr:itm:i}, we have $u \in \stexec(\sigma)$, then 
    from definition of $\stexec$ and $\R'$,
    $\R_{\sigma}(u) \neq \emptyset$ and $\R_{\sigma}(u) = \R'_{a_{\sigma}}(u)$.
    As a consequence, 
    $\R'_{a_{\sigma}}(u) \neq \emptyset$ iff 
    $\R'_{\cset{a_{\sigma}}}(u) \neq \emptyset$, then 
    $u \in \stexec(\cset{a_{\sigma}})$. 
    Thus we can conclude $\truthset{\model_{\modlts}}{\psi} \subseteq \stexec(\strategy)$.

    Now suppose $u \in \R'_{\strategy}(\truthset{\model_{\modlts}}{\psi}) = \R'_{\cset{a_\sigma}}(\truthset{\model_{\modlts}}{\psi})$. By IH, 
    $u \in \R'_{\cset{a_\sigma}}(\truthset{\modlts}{\psi})$.
    Then, by definition of $\R'$, $u \in \R_{\sigma}(\truthset{\modlts}{\psi})$, and by item~\ref{pro2:lr:itm:ii} we have 
    $u \in \truthset{\modlts}{\varphi}$. Then,  
    $u \in \truthset{\model_{\modlts}}{\varphi}$ (by IH), and consequently,
    $\R'_{\strategy}(\truthset{\model_{\modlts}}{\psi}) \subseteq \truthset{\model_{\modlts}}{\varphi}$. 
    
    Therefore, $w \in \truthset{\model_{\modlts}}{\kh(\psi,\varphi)}$.

    %
    % Keep the text below for a long version
    %
    % \begin{enumerate}[\bfseries \itshape (i')]
    %   \item \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
    %           $u \in \truthset{\model_{\modlts}}{\psi}$ & $u \in \truthset{\modlts}{\psi}$                                                 & IH \\
    %                                           & $u \in \stexec(\sigma)$                                                       & \ref{pro2:lr:itm:i} \\
    %                                           & $\R_{\sigma}(u) \neq \emptyset \;\text{and}\; \R_{\sigma} = \R'_{a_{\sigma}}$ & definition of $\mathit{SE}$ and $\R'$ \\
    %                                           & $\R'_{a_{\sigma}}(u) \neq \emptyset$                                          \\
    %                                           & $\R'_{\cset{a_{\sigma}}}(u) \neq \emptyset$                                   \\
    %                                           & $u \in \stexec(\cset{a_{\sigma}})$                                              & definition of $\stexec$ \\
    %                                           & $u \in \stexec(\strategy)$                                                      \\
    %         \end{tabular}
            
    %   Thus, $\truthset{\model_{\modlts}}{\psi} \subseteq \stexec(\strategy)$.
      
    %   \item \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
    %           $u \in \R'_{\strategy}(\truthset{\model_{\modlts}}{\psi})$ & $u \in \R'_{\cset{a_\sigma}}(\truthset{\model_{\modlts}}{\psi})$ \\
    %                                                            & $u \in \R'_{\cset{a_\sigma}}(\truthset{\modlts}{\psi})$   & IH \\
    %                                                            & $u \in \R_{\sigma}(\truthset{\modlts}{\psi})$             & definition of $\R'$ \\
    %                                                            & $u \in \truthset{\modlts}{\varphi}$                       & \ref{pro2:lr:itm:ii} \\
    %                                                            & $u \in \truthset{\model_{\modlts}}{\varphi}$                     & IH \\
    %         \end{tabular}
            
    %   Then, $\R'_{\strategy}(\truthset{\model_{\modlts}}{\psi}) \subseteq \truthset{\model_{\modlts}}{\varphi}$.
    % \end{enumerate}
    % Hence, $w \in \truthset{\model_{\modlts}}{\kh(\psi,\varphi)}$.
    
    \ssparagraph{$\boldsymbol{(\Leftarrow)}$} Suppose
    $w \in \truthset{\model_{\modlts}}{\kh(\psi,\varphi)}$; then there is
    $\strategy \in \S' \subseteq 2^{(\ACT'^*)}$
    satisfying 
    \begin{enumerate}
       \item\label{pro2:rl:itm:i}
      $\truthset{\model_{\modlts}}{\psi} \subseteq \stexec(\strategy)$
      and 
      \item\label{pro2:rl:itm:ii}
      $\R'_\strategy(\truthset{\model_{\modlts}}{\psi}) \subseteq
      \truthset{\model_{\modlts}}{\varphi}$.
    \end{enumerate}
    
    By definition of $\S'$, we have $\strategy = \cset{a_{\sigma}}$
    for some $a_\sigma \in \ACT'$, so
    $\stexec(\sigma) \neq \emptyset$ and $\sigma \in \ACT^*$. Take this
    plan $\sigma$, and suppose $u \in \truthset{\modlts}{\psi}$. By IH,
    $u \in \truthset{\model_{\modlts}}{\psi}$.  Then, we have
    $u \in \stexec(\strategy)$ (by item~\ref{pro2:rl:itm:i}).  By
    definition of $\stexec$ we get $\R'_{\strategy}(u) \neq \emptyset$, iff
    $\R'_{\cset{a_{\sigma}}}(u) \neq \emptyset$.  Then we have
    $\R'_{a_{\sigma}}(u) \neq \emptyset$, which by definition of $\R'$,
    implies $u \in \stexec(\sigma)$.  Thus,
    $\truthset{\modlts}{\psi} \subseteq \stexec(\sigma)$.

    Now take $u \in \R_{\sigma}(\truthset{\modlts}{\psi})$.
    By just applying definitions, it is easy to 
    see that  $u \in \R'_{\strategy}(\truthset{\model_{\modlts}}{\psi})$. Then,
    by item~\ref{pro2:rl:itm:ii}, $u \in \truthset{\model_{\modlts}}{\varphi}$, 
    and by IH, $u \in \truthset{\modlts}{\varphi}$. Thus, $\R_{\sigma}(\truthset{\modlts}{\psi}) \subseteq \truthset{\modlts}{\varphi}$.

    %
    % Keep the text below for a long version
    %
    %\begin{enumerate}[\bfseries \itshape (i')]
    %   \item\label{pro2:rl:itm:ip} \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
    %           $u \in \truthset{\modlts}{\psi}$ & $u \in \truthset{\model_{\modlts}}{\psi}$             & IH \\
    %                                         & $u \in \stexec(\strategy)$                    & \ref{pro2:rl:itm:i} \\
    %                                         & $\R'_{\strategy}(u) \neq \emptyset$         & definition of $\stexec$ \\                                      
    %                                         & $\R'_{\cset{a_{\sigma}}}(u) \neq \emptyset$ \\
    %                                         & $\R'_{a_{\sigma}}(u) \neq \emptyset$        \\
    %                                         & $u \in \stexec(\sigma)$                     & definition of $\R'$ \\
    
    %         \end{tabular}
            
    %   Thus, $\truthset{\modlts}{\psi} \subseteq \stexec(\sigma)$.
    %
    % 
    %   \item \begin{tabular}[t]{@{}l@{\;$\Rightarrow$\;}l@{\quad}l@{}}
    %           $u \in \R_{\sigma}(\truthset{\modlts}{\psi})$ & $u \in \R_{\sigma}(\truthset{\model_{\modlts}}{\psi})$                                  & IH \\
    %                                                      & $u \in \R_{\sigma}(v) \;\text{for some}\; v \in \truthset{\model_{\modlts}}{\psi}$      \\
    %                                                      & $u \in \R'_{a_{\sigma}}(v) \;\text{for some}\; v \in \truthset{\model_{\modlts}}{\psi}$ & \footnotemark \\
    %                                                      & $u \in \R'_{a_{\sigma}}(\truthset{\model_{\modlts}}{\psi})$                             \\
    %                                                      & $u \in \R'_{\cset{a_{\sigma}}}(\truthset{\model_{\modlts}}{\psi})$                      \\
    %                                                      & $u \in \R'_{\strategy}(\truthset{\model_{\modlts}}{\psi})$                              \\
    %                                                      & $u \in \truthset{\model_{\modlts}}{\varphi}$                                            & \ref{pro2:rl:itm:ii} \\
    %                                                      & $u \in \truthset{\modlts}{\varphi}$                                              & IH \\
                                                         

    %         \end{tabular}
    %         \footnotetext{From IH, $v \in \truthset{\model_{\modlts}}{\psi}$ implies $v \in \truthset{\modlts}{\psi}$, which by the just proved Itm \hyperref[pro2:rl:itm:ip]{\ITM{i'}} implies $v \in \stexec(\sigma)$. Then, by definition of $\R'$, we have $\R'_{a_{\sigma}} = \R_{\sigma}$.}
            
    %   Thus, $\R_{\sigma}(\truthset{\modlts}{\psi}) \subseteq \truthset{\modlts}{\varphi}$.
    % \end{enumerate}
    Therefore, we can conclude $w \in \truthset{\modlts}{\kh(\psi,\varphi)}$.
  \end{proof}

  
From these results, we can conclude that the axiom system for $\KHlogic$ over
\lts~\cite{Wang15lori,Wang2016} in Table~\ref{tab:khaxiom} is also sound and complete for $\KHlogic$ over \emph{active} and \emph{compositional} \ultss.
%

\begin{theorem}
\label{th:kh-complete}
The axiom system $\KHaxiom$ (Table~\ref{tab:khaxiom}) is sound and strongly complete w.r.t. the class of active
and compositional \ultss.
\end{theorem}
\begin{proof}
For soundness, let $\model,w$ be an active and compositional pointed \ults. 
By Proposition~\ref{prop:esmtolts}, there exists an \lts $\modlts_{\model}$
s.t. $\model,w\models\varphi$ iff $\modlts_\model,w\models\varphi$,
for all $\varphi$.  Since $\modlts_\model$ is an \lts, and every axiom
$\psi$ in $\KHaxiom$ holds in every \lts,
$\modlts_\model,w\models\psi$. Hence $\model,w\models\psi$, for all
$\psi$ in $\KHaxiom$, i.e., axioms and rules are sound over \ultss.

To prove that $\KHaxiom$ is strongly complete over the class of active and compositional \ults we need to show that, given $\Gamma\cup\cset{\varphi}$ a set of formulas in $\KHlogic$, $\Gamma\models\varphi$ implies $\Gamma\vdash\varphi$. 
  Let $\Gamma$ be a consistent set of formulas. As in~\cite[Lemma
  1]{Wang2016}, $\Gamma$ can be extended to an MCS $\Gamma'$, and as a
  consequence, there exists an LTS $\modlts^{\Gamma'}$ such that
  $\modlts^{\Gamma'},\Gamma'\models\Gamma$ (notice that states in the
  canonical model are MCS). Then, by Proposition~\ref{prop:ltstoesm}, we can
  obtain an \ults $\model_{\modlts^{\Gamma'}}$, such
  that $\model_{\modlts^{\Gamma'}},\Gamma'\models\Gamma$. Moreover,
  from Proposition~\ref{prop:ltstoesm} we know that $\model_{\modlts^{\Gamma'}}$ is
  active and compositional.
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

